Finding the Sweet Spot: Preference Data Construction for Scaling Preference Optimization

Iterative data generation and model retraining are widely used to align large language models (LLMs). It typically involves a policy model to generate on-policy responses and a reward model to guide training data selection. Direct Preference Optimization (DPO) further enhances this process by constructing preference pairs of chosen and rejected responses. In this work, we aim to \emph{scale up} the number of on-policy samples via repeated random sampling to improve alignment performance. Conventional practice selects the sample with the highest reward as chosen and the lowest as rejected for DPO. However, our experiments reveal that this strategy leads to a \emph{decline} in performance as the sample size increases. To address this, we investigate preference data construction through the lens of underlying normal distribution of sample rewards. We categorize the reward space into seven representative points and systematically explore all 21 ($C_7^2$) pairwise combinations. Through evaluations on four models using AlpacaEval 2, we find that selecting the rejected response at reward position $\mu - 2\sigma$ rather than the minimum reward, is crucial for optimal performance. We finally introduce a scalable preference data construction strategy that consistently enhances model performance as the sample scale increases.

==> figuretexs/bar_freq.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=0.8\linewidth]{figs/bar_0.25.pdf}
\vspace{0.5em} % Add spacing between images
\includegraphics[width=0.8\linewidth]{figs/bar_0.5.pdf}
\vspace{0.5em} % Add spacing between images
\includegraphics[width=0.8\linewidth]{figs/bar_0.75.pdf}
\caption{Frequency of prompts where the $\frac{1}{4}$, $\frac{1}{2}$, and $\frac{3}{4}$ response reward points fall within different intervals of the normal distribution.}
\label{bar_freq}
\end{figure}


==> figuretexs/mistral_loss.tex <==
\begin{figure*}[!ht]
\centering
\includegraphics[width=0.95\linewidth]{figs/mistral_loss.pdf}
\caption{}
\label{mistral_loss}
\vspace{-1em}
\end{figure*}

==> figuretexs/normal.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=0.8\linewidth, clip=true, trim = 55mm 10mm 40mm 5mm]{figs/normal.pdf}
\caption{}
\label{normal}
\vspace{-1em}
\end{figure}

==> figuretexs/pipe.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=1\linewidth, clip=true, trim = 75mm 83mm 79mm 46mm]{figs/main_illu_first.pdf}
\caption{The upper part shows the pipeline of preference data construction; the middle part show a conventional strategy of preference data construction, which leads to decline of performance with increasing number fo samples; the lower part shows the focus of this paper, and our proposed simple approach.}
\label{pipe}
\vspace{-1em}
\end{figure}

==> figuretexs/reject_u_-2sigma.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=0.6\linewidth]{figs/llamainstruct_reject_mu_-2sigma.pdf}
\caption{When the rejected response is appropriately selected for DPO, the performance of the trained models will improve as the chosen response is getting better. x-axis is the reward position where the chosen response is selected, y-axis is the score (\%).}
\label{rejected_mu_-2sgima}
\vspace{-1em}
\end{figure}

==> tabletex/extend_point.tex <==
\begin{table}[!t]
\centering
\resizebox{0.33\textwidth}{!}{
\begin{tabular}{l l c c }
\toprule
\multirow{2}{*}{\textbf{Chosen}} & \multirow{2}{*}{\textbf{Rejected}} & \multicolumn{2}{c}{\textbf{Llama-Inst}} \\
\cmidrule(lr){3-4} & & \textbf{LC} & \textbf{WR} \\
\midrule         
$max$          & $min$                              & 43.11      & 43.97         \\
\midrule
$max$          & $\mu-4\sigma$                      & 43.61      & 44.30         \\
$max$          & $\mu-3\sigma$                      & 44.10      & 43.78         \\
\midrule
$max$          & $\mu-2\sigma$                      & 48.12      & 49.66                \\
\midrule
$\mu+4\sigma$  & $\mu-2\sigma$                      & 48.11      & 49.46         \\
$\mu+3\sigma$  & $\mu-2\sigma$                      & 48.26      & 49.20         \\
\bottomrule
\end{tabular}
}
\caption{}
\label{wide_scale}
\vspace{-1em}
\end{table}

==> tabletex/hyperparam.tex <==



==> tabletex/instruct.tex <==
% \begin{table*}[!t]
% \centering
% \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{l l c c c c c c c c c c}
% \toprule
% \multirow{2}{*}{\textbf{Chosen}} & \multirow{2}{*}{\textbf{Rejected}} & \multicolumn{2}{c}{\textbf{Llama-Base}} & \multicolumn{2}{c}{\textbf{Mistral-Base}} & \multicolumn{2}{c}{\textbf{Llama-Inst}} & \multicolumn{2}{c}{\textbf{Mistral-Inst}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
% & & \textbf{LC} & \textbf{WR} & \textbf{LC} & \textbf{WR} & \textbf{LC} & \textbf{WR} & \textbf{LC} & \textbf{WR} \\
% \midrule
% max\_of\_5      & min\_of\_5    & 16.58      & 11.29      & 81.30       & 32.95       & 83.10       & 38.22       & 82.50       & 36.90       \\
% \midrule
% max             & min           & 16.42      & 10.99      & 81.30       & 32.95       & 82.90       & 38.01       & 82.10       & 36.50       \\
% max             & $\mu-2\sigma$ & 19.07      & 13.67      & 82.20       & 36.38       & 84.20       & 40.15       & 83.40       & 38.40       \\
% max             & $\mu-\sigma$  & 18.58      & 15.43      & 82.90       & 37.13       & 83.87       & 39.72       & 83.10       & 37.90       \\
% max             & $\mu$         & 17.78      & 16.06      & 82.90       & 37.13       & 83.60       & 39.15       & 82.90       & 37.50       \\
% max             & $\mu+\sigma$  & 17.58      & 17.16      & 82.90       & 37.13       & 83.25       & 38.85       & 82.60       & 37.20       \\
% max             & $\mu+2\sigma$ & 10.58      & 9.08       & 82.90       & 37.13       & 81.90       & 35.50       & 81.30       & 35.10       \\
% $\mu+2\sigma$   & min           & 14.82      & 10.17      & 82.90       & 37.13       & 82.10       & 36.11       & 81.50       & 35.60       \\
% $\mu+2\sigma$   & $\mu-2\sigma$ & 19.45      & 13.27      & 82.90       & 37.13       & 84.30       & 40.35       & 83.50       & 38.70       \\
% $\mu+2\sigma$   & $\mu-\sigma$  & 18.85      & 14.71      & 82.90       & 37.13       & 83.90       & 39.80       & 83.20       & 38.20       \\ 
% $\mu+2\sigma$   & $\mu$         & 18.55      & 16.22      & 82.90       & 37.13       & 83.70       & 39.35       & 83.00       & 37.80       \\
% $\mu+2\sigma$   & $\mu+\sigma$  & 15.86      & 15.36      & 82.90       & 37.13       & 82.80       & 38.12       & 82.40       & 37.00       \\
% $\mu+\sigma$    & min           & 14.08      & 8.41       & 82.90       & 37.13       & 82.30       & 37.21       & 81.70       & 36.20       \\
% $\mu+\sigma$    & $\mu-2\sigma$ & 17.62      & 10.96      & 82.90       & 37.13       & 83.00       & 38.47       & 82.60       & 37.10       \\
% $\mu+\sigma$    & $\mu-\sigma$  & 17.53      & 11.52      & 82.90       & 37.13       & 82.90       & 38.33       & 82.50       & 36.90       \\
% $\mu+\sigma$    & $\mu$         & 14.83      & 11.21      & 82.90       & 37.13       & 82.70       & 38.00       & 82.30       & 36.70       \\
% $\mu$           & min           & 11.68      & 6.39       & 82.90       & 37.13       & 81.50       & 35.90       & 81.20       & 35.40       \\
% $\mu$           & $\mu-2\sigma$ & 14.31      & 8.25       & 82.90       & 37.13       & 82.00       & 36.45       & 81.70       & 36.10       \\
% $\mu$           & $\mu-\sigma$  & 15.00      & 9.21       & 82.90       & 37.13       & 82.10       & 36.80       & 81.80       & 36.20       \\
% $\mu-\sigma$    & min           & 9.17       & 5.27       & 82.90       & 37.13       & 80.90       & 35.40       & 80.60       & 35.00       \\
% $\mu-\sigma$    & $\mu-2\sigma$ & 10.97      & 6.29       & 82.90       & 37.13       & 81.00       & 35.65       & 80.70       & 35.20       \\
% $\mu-2\sigma$   & min           & 9.47       & 5.25       & 82.90       & 37.13       & 80.70       & 35.20       & 80.40       & 34.90       \\

% \bottomrule
% \end{tabular}
% }
% \caption{Skywork (\%).}
% \label{results_main_skywork}
% \vspace{-1em}
% \end{table*}





\begin{table}[!t]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l l c c c c c c}
\toprule
\multirow{2}{*}{\textbf{Chosen}} & \multirow{2}{*}{\textbf{Rejected}} & \multicolumn{2}{c}{\textbf{Llama-Base}} & \multicolumn{2}{c}{\textbf{Mistral-Base}}  \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} 
& & \textbf{LC} & \textbf{WR} & \textbf{LC} & \textbf{WR} \\
\midrule
max\_of\_5      & min\_of\_5    & 16.58      & 11.29      & 81.30       & 32.95              \\
\midrule
max             & min           & 16.42      & 10.99      & 81.30       & 32.95              \\
max             & $\mu-2\sigma$ & 19.07      & 13.67      & 82.20       & 36.38             \\
max             & $\mu-\sigma$  & 18.58      & 15.43      & 82.90       & 37.13              \\
max             & $\mu$         & 17.78      & 16.06      & 82.90       & 37.13             \\
max             & $\mu+\sigma$  & 17.58      & 17.16      & 82.90       & 37.13             \\
max             & $\mu+2\sigma$ & 10.58      & 9.08       & 82.90       & 37.13             \\
$\mu+2\sigma$   & min           & 14.82      & 10.17      & 82.90       & 37.13           \\
$\mu+2\sigma$   & $\mu-2\sigma$ & 19.45      & 13.27      & 82.90       & 37.13            \\
$\mu+2\sigma$   & $\mu-\sigma$  & 18.85      & 14.71      & 82.90       & 37.13              \\ 
$\mu+2\sigma$   & $\mu$         & 18.55      & 16.22      & 82.90       & 37.13              \\
$\mu+2\sigma$   & $\mu+\sigma$  & 15.86      & 15.36      & 82.90       & 37.13             \\
$\mu+\sigma$    & min           & 14.08      & 8.41       & 82.90       & 37.13            \\
$\mu+\sigma$    & $\mu-2\sigma$ & 17.62      & 10.96      & 82.90       & 37.13            \\
$\mu+\sigma$    & $\mu-\sigma$  & 17.53      & 11.52      & 82.90       & 37.13            \\
$\mu+\sigma$    & $\mu$         & 14.83      & 11.21      & 82.90       & 37.13             \\
$\mu$           & min           & 11.68      & 6.39       & 82.90       & 37.13          \\
$\mu$           & $\mu-2\sigma$ & 14.31      & 8.25       & 82.90       & 37.13             \\
$\mu$           & $\mu-\sigma$  & 15.00      & 9.21       & 82.90       & 37.13             \\
$\mu-\sigma$    & min           & 9.17       & 5.27       & 82.90       & 37.13              \\
$\mu-\sigma$    & $\mu-2\sigma$ & 10.97      & 6.29       & 82.90       & 37.13           \\
$\mu-2\sigma$   & min           & 9.47       & 5.25       & 82.90       & 37.13           \\

\bottomrule
\end{tabular}
}
\caption{Armorm (\%).}
\label{results_main_skywork}
\vspace{-1em}
\end{table}

